Double Oracle Neural Architecture Search for Game Theoretic Deep Learning Models

In this paper, we propose a new approach to train deep learning models using game theory concepts including Generative Adversarial Networks (GANs) and Adversarial Training (AT) where we deploy a double-oracle framework using best response oracles. GAN is essentially a two-player zero-sum game between the generator and the discriminator. The same concept can be applied to AT with attacker and classifier as players. Training these models is challenging as a pure Nash equilibrium may not exist and even finding the mixed Nash equilibrium is difficult as training algorithms for both GAN and AT have a large-scale strategy space. Extending our preliminary model DO-GAN, we propose the methods to apply the double oracle framework concept to Adversarial Neural Architecture Search (NAS for GAN) and Adversarial Training (NAS for AT) algorithms. We first generalize the players' strategies as the trained models of generator and discriminator from the best response oracles. We then compute the meta-strategies using a linear program. For scalability of the framework where multiple network models of best responses are stored in the memory, we prune the weakly-dominated players' strategies to keep the oracles from becoming intractable. Finally, we conduct experiments on MNIST, CIFAR-10 and TinyImageNet for DONAS-GAN. We also evaluate the robustness under FGSM and PGD attacks on CIFAR-10, SVHN and TinyImageNet for DONAS-AT. We show that all our variants have significant improvements in both subjective qualitative evaluation and quantitative metrics, compared with their respective base architectures.

==> Content/Body/TerminationCheckAlgo.tex <==
\begin{algorithm}
\caption{$\mathtt{Termination Check}(U^{t}, \sigma^{t*}_{p1}, \sigma^{t*}_{p2})$}
\begin{algorithmic}[1]
\STATE Compute $U^{t}(\sigma^{t*}_{p1},\sigma^{t*}_{p2})$; \\
// $U^{t}$ is of size $m \times n$ \label{findUstart}
\STATE Compute $U^{t}(\sigma^{t*}_{p1}, \mathcal{P}_{2}[n])$; \\ 
// $|\mathcal{P}_{1}|=m, |\mathcal{P}_{2}|=n$
\STATE Compute $U^{t}(\mathcal{P}_{1}[m], \sigma^{t*}_{p2})$; \label{findUend} 
\STATE $\delta_{p_{1}} = U^{t}(\mathcal{P}_{1}[m], \sigma^{t*}_{p2}) - U^{t}(\sigma^{t*}_{p1}, \sigma^{t*}_{p2})$; \label{gendiff}
\STATE $\delta_{p_{2}} = U^{t}(\sigma^{t*}_{p1}, \sigma^{t*}_{p2})-U^{t}(\sigma^{t*}_{p1}, \mathcal{P}_{2}[n])$\label{disDiff};
\IF{$\delta_{p_{1}} < \epsilon~\&\&~-\delta_{p_{2}} < \epsilon$  \label{diffStart}}
\STATE \textbf{return True}
\ELSE
\STATE \textbf{return False}  \label{diffEnd}
\ENDIF
\end{algorithmic}
\label{TerminationCheck}
\end{algorithm}



==> Content/Body/dogan.tex <==
As discussed in previous sections, computing mixed NE for AML is challenging as there is an extremely large number of pure strategies, i.e., possible parameter settings of the trained networks i.e., generator, discriminator or classifier. Thus, we propose a double oracle frameworks for AML consisting of pure GAN (DO-GAN), Adversarial-Neural Architecture Search (DONAS-GAN) and Neural Architecture Search for Adversarial Training (DONAS-AT) to compute the mixed NE efficiently. Over the different AML methods, the DO framework builds a restricted meta-matrix game between the two players and computes the mixed NE of the meta-matrix game, then iteratively adds more strategies of the two players (generators/discriminators or classifier/attacker) into the meta-matrix game until termination.

\subsection{General Framework of DO-GAN}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{Content/Figures/do-gan-xscale.pdf}
    \caption{An illustration of Double Oracle Framework for Adversarial Machine Learning. Figure adapted from~\cite{lanctot2017unified}.}
    \label{fig:illustrative_do_gan}
\end{figure*}

GAN can be translated as a two-player zero-sum game between the generator player $g$ and the discriminator player $d$. To compute the mixed NE of GANs, at iteration $t$, DO-GAN creates a restricted meta-matrix game $U^{t}$ with the trained generators and discriminators as strategies of the two players, where the generators and discriminators are parameterized by $\pi_{g}\in\mathcal{G}$ and $\pi_{d}\in\mathcal{D}$. We use $U^{t}(\pi_{g}, \pi_{d})$ to denote the generator player's payoff when playing $\pi_{g}$ against $\pi_{d}$, which is defined as $L_{D}$. Since GAN is zero-sum, the discriminator player's payoff is $-U^{t}(\pi_{g}, \pi_{d})$. We define $\sigma^{t}_{g}$ and $\sigma^{t}_{d}$ as the mixed strategies of generator player and discriminator player, respectively. With a slight abuse of notation, we define the generator player's expected utility of mixed strategies $\langle\sigma^{t}_{g},\sigma^{t}_{d}\rangle$ as $U^{t}(\sigma^{t}_{g}, \sigma^{t}_{d}) = \sum_{\pi_{g} \in \mathcal{G}} \sum_{\pi_{d} \in \mathcal{D}} \sigma^{t}_g(\pi_{g}) \cdot \sigma^{t}_{d}(\pi_{d}) \cdot U^{t}(\pi_{g},\pi_{d})$. We use $\langle\sigma_{g}^{t*},\sigma_{d}^{t*}\rangle$ to denote mixed NE of the restricted meta-matrix game $U^{t}$. We solve $U^{t}$ to obtain the mixed NE, compute best responses and add them into $U^{t}$ for next iteration. Figure~\ref{fig:illustrative_do_gan} presents an illustration of DO-GAN and Algorithm~\ref{dogan} describes the overview of the framework. 

Our algorithm starts by initializing two arrays $\mathcal{G}$ and $\mathcal{D}$ to store multiple generators and discriminators (line~\ref{initializeGD}). We train the first $\pi_{g}$ and $\pi_{d}$ with the canonical training procedure of GANs (line~\ref{trainCoreStart}). We store the parameters of trained models in $\mathcal{G}$ and $\mathcal{D}$ (line~\ref{assignmodels}), compute the adversarial loss $L_{D}$ and add it to the meta-matrix $U^{0}$ (line~\ref{computepayofffirst}). We initialize the meta-strategies $\sigma^{0*}_g=[1]$ and $\sigma^{0*}_d=[1]$ since there is only one pair of generator and discriminator available (line~\ref{initializeSigma}). For each epoch, we use $\mathtt{generatorOracle()}$ and $\mathtt{discriminatorOracle()}$ to obtain best responses $\pi'_{g}$ and $\pi'_{d}$ to $\sigma^{t*}_{d}$ and $\sigma^{t*}_{g}$ via Adam Optimizer, respectively, then add them into $\mathcal{G}$ and $\mathcal{D}$ (lines~\ref{bestresponseGStart}-\ref{bestresponseDEnd}). We then augment $U^{t-1}$ by adding $\pi'_{g}$ and $\pi'_{d}$ and calculating $U^{t}(\pi'_{g}, \pi'_{d})$ to obtain $U^{t}$ and compute the missing entries (line~\ref{payoffCompute}). We compute the missing payoff entries $U^{t}(\pi'_{g}, \pi_{d}), \forall \pi_{d} \in \mathcal{D}$ and $U^{t}(\pi_{g}, \pi'_{d}), \forall \pi_{g} \in \mathcal{G}$ by sampling a few batches of training data. After that, we compute the mixed NE $\langle\sigma_{g}^{t*},\sigma_{d}^{t*}\rangle$ of $U^{t}$ with linear programming (line~\ref{lp}). The algorithm terminates if the criteria described in Algorithm~\ref{term} is satisfied (line~\ref{terminationCheck}). 

%We also prune the support strategy set of the players as described in Algorithm~\ref{prune} (line~\ref{pruning}) to avoid $\mathcal{G}$ and $\mathcal{D}$ becoming intractable.

In $\mathtt{generatorOracle}()$, we train $\pi'_{g}$ to obtain the best response against $\sigma^{t*}_{d}$, i.e., $U^{t}(\pi'_{g}, \sigma^{t*}_{d}) \geq U^{t}(\pi_{g}, \sigma^{t*}_{d}), \forall \pi_{g} \in \Pi_{g}$. Similarly, in $\mathtt{disciminatorOracle}()$, we train $\pi'_{d}$ to obtain the best response against $\sigma^{t*}_{g}$, i.e., $U^{t}(\sigma^{t*}_{g}, \pi'_{d}) \geq U^{t}(\sigma^{t*}_{g}, \pi_{d}), \forall \pi_d \in \Pi_{d}$. Full details of generator oracle and discriminator oracle can be found in Appendix~\ref{appendixA}.

\begin{algorithm}
\small
\DontPrintSemicolon
%Double Oracle Framework for GAN (
\caption{$\mathtt{DO-GAN()}$}
\label{dogan}
\SetKwInOut{Input}{input}
\SetKwComment{Comment}{//\ }{}
 \newcommand\mycommfont[1]{\footnotesize{#1}}
\SetCommentSty{mycommfont}
  Initialize generator and discriminator arrays $\mathcal{G} = \emptyset$ and $\mathcal{D} = \emptyset$; \label{initializeGD}\par
    Train generator \& discriminator to get the first $\pi_{g}$ and $\pi_{d}$; \label{trainCoreStart}   \par
  $\mathcal{G} \leftarrow \mathcal{G} \cup \{\pi_{g}\}$; $\mathcal{D} \leftarrow \mathcal{D} \cup \{\pi_{d}\}$; \label{assignmodels}\par
  Compute the adversarial loss $L_{D}$ and add it to meta-matrix $U^{0}$; \label{computepayofffirst}\par
  Initialize $\sigma^{0*}_g =[1]$ and $\sigma^{0*}_d=[1]$; \label{initializeSigma}\par
  \For{epoch $t \in \{1,2,...\}$}{
         $\pi'_{g} \leftarrow \mathtt{generatorOracle}(\sigma_{d}^{t*}, \mathcal{D})$; \label{bestresponseGStart}\par
        $\mathcal{G} \leftarrow \mathcal{G} \cup \{\pi'_{g}\}$; \label{bestresponseGEnd}\par
         $\pi'_{d} \leftarrow \mathtt{discriminatorOracle}(\sigma_{g}^{t*}, \mathcal{G})$;\label{bestresponseDStart} \par
        $\mathcal{D} \leftarrow \mathcal{D} \cup \{\pi'_{d}\}$; \par \label{bestresponseDEnd}\par
        Augment $U^{t-1}$ with $\pi'_{g}$ and $\pi'_{d}$ to obtain $U^{t}$ and compute missing entries; \label{payoffCompute} \par
       Compute mixed NE $\langle\sigma^{t*}_g, \sigma^{t*}_d\rangle$ for $U^{t}$ with linear program; \label{lp} \Comment*[r]{Section~\ref{lpMM}}
         \lIf(\hfill// \small{Section~\ref{termcheck}}){\texttt{\emph{TerminationCheck($U^{t}, \sigma^{t*}_g, \sigma^{t*}_d$)}
             \label{terminationCheck}}}{ 
            \textbf{break};
         } 
      }
\end{algorithm}

\subsection{Linear Program for Meta-matrix Game} \label{lpMM}
Since the current restricted meta-matrix game $U^{t}$ is a zero-sum game, we can use a linear program to compute the mixed NE in polynomial time~\cite{schrijver1998theory}.
Given the generator player $g$'s mixed strategy $\sigma^{t}_{g}$, the discriminator player $d$ will play strategies that minimize the expected utility of $g$. Thus, the mixed NE strategy for the generator player $\sigma^{t*}_{g}$ is to maximize the worst-case expected utility, which is obtained by solving the following linear program: 
\begin{multline}
    \sigma^{t*}_{g} = \arg \max\nolimits_{\sigma^{t}_{g}} \{v: \sigma^{t}_{g} \geq 0, \sum\nolimits_{i \in \mathcal{G}} \sigma^{t}_{g}(i) = 1, \\ U^{t}(\sigma^{t}_{g}, \pi_{d}) \geq v, \forall \pi_{d} \in \mathcal{D}\}.
    \label{lpeq}
\end{multline}
Similarly, we can obtain the mixed NE strategy for the discriminator $\sigma_{d}^{t*}$ by solving a linear program that maximizes the worst-case expected utility of the discriminator player. Therefore, we obtain the mixed NE $\langle\sigma^{t*}_{g}, \sigma^{t*}_{d}\rangle$ of the restricted meta-matrix game $U^{t}$.

\subsection{Termination Check}\label{termcheck}
DO terminates the training by checking whether the best response $\pi'_{g}$ (or $\pi'_{d}$) is in the support set $\mathcal{G}$ (or $\mathcal{D}$)~\cite{jain2011double}, but we cannot apply this approach to DO-GAN as GAN has infinite-dimensional strategy space~\cite{hsieh2018finding}.
Hence, we terminate the training if the best responses cannot bring a higher utility to the two players than the entries of the current support sets, as discussed in~\cite{lanctot2017unified,muller2019generalized}. Specifically, we first compute $U^{t}(\sigma^{t*}_{g}, \sigma^{t*}_{d})$ and the expected utilities for new generator and discriminator $U^{t}(\mathcal{G}[m], \sigma^{t*}_{d}), U^{t}(\sigma^{t*}_{g}, \mathcal{D}[n])$ (line~\ref{findUstart}-\ref{findUend}). Then, we calculate the utility increment (lines~\ref{gendiff}-\ref{disDiff}) and returns \textbf{True} if both $U^{t}(\mathcal{G}[m], \sigma^{t*}_{d})$ and $ U^{t}(\sigma^{t*}_{g}, \mathcal{D}[n])$ cannot bring a higher utility than $U^{t}(\sigma^{t*}_{g},\sigma^{t*}_{d})$ by $\epsilon$ (lines~\ref{diffStart}-\ref{diffEnd}).

\begin{algorithm}
\small
\caption{$\mathtt{Termination Check}(U^{t}, \sigma^{t*}_{g}, \sigma^{t*}_{d})$}
 \label{term}
\SetKwInOut{Input}{input}
\SetKwComment{Comment}{//\ }{}
 \newcommand\mycommfont[1]{\footnotesize{#1}}
\SetCommentSty{mycommfont}
\Comment{$U^{t}$ is of size $m \times n$}
\Comment{$|G|=m, |D|=n$}
Compute $U^{t}(\sigma^{t*}_{g},\sigma^{t*}_{d})$; \label{findUstart} \par
Compute $U^{t}(\sigma^{t*}_{g}, \mathcal{D}[n])$; \par
Compute $U^{t}(\mathcal{G}[m], \sigma^{t*}_{d})$; \label{findUend} \par
$\textit{genInc} = U^{t}(\mathcal{G}[m], \sigma^{t*}_{d}) - U^{t}(\sigma^{t*}_{g}, \sigma^{t*}_{d})$;\par \label{gendiff}
$\textit{disInc} = -U^{t}(\sigma^{t*}_{g}, \mathcal{D}[n]) -(- U^{t}(\sigma^{t*}_{g}, \sigma^{t*}_{d}))$; \par  \label{disDiff}
    \If{$\text{genInc} < \epsilon~\&\&~-\text{disInc} < \epsilon$  \label{diffStart}}{ 
    \Return\textbf{True}
}
\lElse{
    \Return\textbf{False} 
} \label{diffEnd}
\end{algorithm}

\begin{algorithm}
\small
%\caption{$\mathtt{PruneMetaMatrix}(U^{t}, \sigma^{t*}_{g}, \sigma^{t*}_{d})$}
\caption{DO-GAN/P}
 \label{prune}
\SetKwInOut{Input}{input}
\SetKwComment{Comment}{//\ }{}
 \newcommand\mycommfont[1]{\footnotesize{#1}}
\SetCommentSty{mycommfont}\
\Comment{I stores indices to be pruned from $\mathcal{G}$ and $\mathcal{D}$}
\Comment{G stores models to be pruned from $\mathcal{G}$ and $\mathcal{D}$}
$\mathtt{DO-GAN()}$;\par
$I_{g}=\emptyset; I_{d} = \emptyset$ \par
$K_{g}=\emptyset; K_{d}=\emptyset$ 
\If{$|\mathcal{G}| > s$ \label{pruneStart}}{
    \For{$i \in \{0, \dots, |\mathcal{G}|-1\}$}{
        \lIf{$\sigma^{t*}_{g}(\mathcal{G}[i]) == \min \sigma^{t*}_{g}$}{
            $I_{g} \leftarrow I_{g} \cup \{i\}$;
            $K_{g} \leftarrow K_{g} \cup \{\mathcal{G}[i]\}$
        }
    }
    }
    \If{$|\mathcal{D}| > s$}{
    \For{$j \in \{0, \dots, |\mathcal{D}|-1\}$}{
        \lIf{$\sigma^{t*}_{d}(\mathcal{D}[j]) == \min \sigma^{t*}_{d}$}{
            $I_{d} \leftarrow I_{d} \cup \{j\} $; 
            $K_{d} \leftarrow K_{d} \cup \{\mathcal{D}[j]\}$
        }
    }
    } 
    $\mathcal{G} \leftarrow \mathcal{G} \setminus K_{g}$; 
    $\mathcal{D} \leftarrow \mathcal{D} \setminus K_{d}$; \label{pruneEnd}\par
    $U \leftarrow J_{I_{g}, m} \cdot U^{t} \cdot J^{T}_{I_{d},n}$ \label{pruneU}
\end{algorithm}

\begin{algorithm}
\small
\DontPrintSemicolon
\caption{DO-GAN/C}
\label{contdogan}
\SetKwInOut{Input}{input}
\SetKwComment{Comment}{//\ }{}
 \newcommand\mycommfont[1]{\footnotesize{#1}}
\SetCommentSty{mycommfont}
  Initialize generator and discriminator task arrays $\mathcal{G} = \emptyset$ and $\mathcal{D} = \emptyset$; \label{initializeGDcont}\par
    Train generator \& discriminator to get with the first task to get $\pi^{0}_{g}$ and $\pi^{0}_{d}$; \label{trainCoreStartcont}   \par
  $\mathcal{G} \leftarrow \mathcal{G} \cup \{\pi_{g}\}$; $\mathcal{D} \leftarrow \mathcal{D} \cup \{\pi_{d}\}$; \label{assignmodelscont}\par
  Compute the adversarial loss $L_{D}$ and add it to meta-matrix $U^{0}$; \label{computepayofffirstcont}\par
  Initialize $\sigma^{0*}_g =[1]$ and $\sigma^{0*}_d=[1]$; \label{initializeSigmacont}\par
  \For{epoch $t \in \{1,2,...\}$}{
        Create new tasks $\pi^{t}_{g}$ and $\pi^{t}_{d}$; \label{createTask}\par
         $\pi^{t}_{g} \leftarrow \mathtt{generatorOracle}(\sigma_{d}^{t*}, \mathcal{D})$; \label{bestresponseGStartcont}\par
        $\mathcal{G} \leftarrow \mathcal{G} \cup \{\pi^{t}_{g}\}$; \label{bestresponseGEndcont}\par
         $\pi^{t}_{d} \leftarrow \mathtt{discriminatorOracle}(\sigma_{g}^{t*}, \mathcal{G})$;\label{bestresponseDStartcont} \par
        $\mathcal{D} \leftarrow \mathcal{D} \cup \{\pi^{t}_{d}\}$; \par \label{bestresponseDEndcont}\par
        \If{$t \geq 2$}{$\mathcal{G}\setminus \{ \pi^{t-2}_{g} \}$ \text{ and } $\mathcal{D} \setminus \{ \pi^{t-2}_{d} \}$ ;\label{removeprevious}}
        Create $U^{t}$ with $\pi^{t-1}_{g}, \pi^{t}_{g}$ and $\pi^{t-1}_{d}, \pi^{t}_{d}$; \label{payoffComputecont} \par
       Compute mixed NE $\langle\sigma^{t*}_g, \sigma^{t*}_d\rangle$ for $U^{t}$ with linear program; \label{lpcont} \Comment*[r]{Section~\ref{lpMM}}
         \lIf(\hfill// \small{Section~\ref{termcheck}}){\texttt{\emph{TerminationCheck($U^{t}, \sigma^{t*}_g, \sigma^{t*}_d$)}
             \label{terminationCheckcont}}}{ 
            \textbf{break};
         } 
      }
\end{algorithm}

==> Content/Body/practicalImplementations.tex <==
\section{Practical Implementations}
As the number of epochs grows during the training of DO, the number of networks and the size of the meta-matrix also grows. Hence, there is a risk that the support strategy set becomes very large and $\mathcal{G}$ and $\mathcal{D}$ become intractable. To make the algorithm practical and scalable, we propose two methods: DO-GAN with meta-matrix pruning (DO-GAN/P) and DO-GAN with continual learning (DO-GAN/C).
\subsection{Meta-matrix Pruning  (DO-GAN/P)}\label{pruneMM}
The first method is to prune the meta-matrix. Here, we adapt the greedy pruning algorithm, as depicted in Algorithm~\ref{prune}. When either $|\mathcal{G}|$ or $|\mathcal{D}|$ is greater than the limit of the support set size $s$, we prune at least one strategy with the least probability, which is the strategy that contributes the least to the player's winning.
Specifically, we define $J_{I,b}$ where $I$ is the set of row numbers to be removed, $b$ is the total rows of a matrix. To remove the $2^{nd}$ row of a matrix having $3$ rows, we define $I= \{1\}, b=3$ and $J_{\{1\},3} =\left( \begin{matrix} 1 & 0 & 0  \\ 0 & 0 & 1  \end{matrix} \right)$. If $|\mathcal{G}|>s$, at least one strategy with minimum probability is pruned from $\mathcal{G}$, similarly for $\mathcal{D}$ (lines~\ref{pruneStart}-\ref{pruneEnd}). Finally, we prune the meta-matrix using matrix multiplication (line~\ref{pruneU}). 

\iffalse
\begin{algorithm}
\small
\caption{DO-GAN/P}
 \label{doganprune}
 \SetKwInOut{Input}{input}
\SetKwComment{Comment}{//\ }{}
 \newcommand\mycommfont[1]{\footnotesize{#1}}
\SetCommentSty{mycommfont}\
        $\mathtt{DO-GAN()}$; \par
        \texttt{PruneMetaMatrix($U^{t}, \sigma^{t*}_g, \sigma^{t*}_d$)}; \label{pruning} 
\end{algorithm}
\fi

\subsection{Continual Learning (DO-GAN/C)}
\label{sec:do_gan_c}
Our ablation studies show that we still need a support set of at least $s=10$ for DO-GAN/P to converge and the time complexity grows as $s$ increases. Thus, we further reduce both time and space complexity by making the network retain the knowledge of previous networks so that the algorithm will converge with even smaller support set. Hence, we propose to adapt continual learning to consolidate the knowledge of multiple networks to a single network while setting $s=2$ to reduce the space complexity as much as possible. We treat each network as a task to train the adaptive continual learning network while having a distribution over the tasks to represent the player's strategies. 

To remedy the catastrophic forgetting i.e., all the generator tasks focus only towards fooling the newest discriminator, we adapt Elastic Weight Consolidation (EWC) method~\cite{li2020few}. We change the generator loss function from non-saturating to saturating and add a penalty function accordingly. Let $G$ be trained on task $t-1$ to have optimal parameters $\pi^{t-1}_{g}$, the Fisher information $F$ is:
\begin{equation}
F = \mathbb{E}_{\mathbf{z} \sim p(\mathbf{z})} \Bigg[\Big(\frac{\delta}{\delta \pi^{t-1}_{g}} \log D(G(\mathbf{z})|\pi^{t-1}_{g})\Big)^{2} \Bigg]
 \end{equation}
 After obtaining the Fisher information, we directly use $F$ as a regularization loss to penalize the weight change during the training. Hence, $G$'s loss function is augmented as:
 \begin{multline}
 L_{G} = \mathbb{E}_{\mathbf{z} \sim p_{\mathbf{z}}(\mathbf{z})}[-\log D(G(\mathbf{z}) \\ + \lambda \cdot \sigma^{t*}_{g} \cdot \sum \nolimits_{i} F_{i} (\pi_{i} - \pi^{t-1,i}_{g})^{2}
\end{multline}
where $\pi^{t-1}_{g}$ represents the parameters learned for task $t-1$, $i$ is the index of each parameter of the generator model, and $\lambda$ is the regularization weight.
 

 
Algorithm \ref{contdogan} describes the changes to $\mathtt{DO-GAN}$ algorithm with continual learning. Instead of arrays $\mathcal{G}$ and $\mathcal{D}$ in $\mathtt{DO-GAN}$, we initialize tasks arrays for generator and discriminator (line \ref{initializeGDcont}). At every epoch, we create new tasks and train the generator and discriminator networks to outperform the previous optimal parameters with the distribution at NE $\sigma_{d}^{t*}$ and $\sigma_{g}^{t*}$ respectively (lines \ref{createTask}-\ref{bestresponseDEndcont}). Then, we keep the previously and currently trained optimal parameters (line \ref{removeprevious}) to create meta-matrix, solve it to compute mixed-NE (lines \ref{payoffComputecont}-\ref{lpcont}). Finally, we perform the termination check (line \ref{terminationCheckcont}).

\begin{theorem}
Given the same architectures, the space complexity of DO-GAN is $\mathcal{O}(t)$ where $t$ is the number of epochs until convergence. In contrast, the space complexity of DO-GAN/P is $\mathcal{O}(s)$ where $s$ is the size of the support set. DO-GAN/C has the minimum storage complexity which is $\mathcal{O}(1)$.
\end{theorem}

In DO-GAN, we add a pair of generator and discriminator for every epoch of training. Thus, the space complexity of DO-GAN is $\mathcal{O}(t)$, making the algorithm memory-inefficient to train with real-world datasets where it needs a large number of epochs to converge. The space complexity of DO-GAN/P is $\mathcal{O}(s)$ since we prune the meta-matrix and the players' strategies if the $|\mathcal{G}|>s$ or $|\mathcal{D}|>s$ where $s$ is the limit of the support set size. In DO-GAN/C, we train a single adaptive network storing the optimal strategies only for the tasks created at $(t-1)^{th}$ and $t^{th}$ epochs. Thus, the space complexity of DO-GAN/C is kept at $\mathcal{O}(1)$.
